Enabling Cognitive Intelligence Queries in Relational Databases using Low-dimensional Word Embeddings

We apply distributed language embedding methods from Natural Language Processing to assign a vector to each database entity associated token (for example, a token may be a word occurring in a table row, or the name of a column). These vectors, of typical dimension 200, capture the meaning of tokens based on the contexts in which the tokens appear together. To form vectors, we apply a learning method to a token sequence derived from the database. We describe various techniques for extracting token sequences from a database. The techniques differ in complexity, in the token sequences they output and in the database information used (e.g., foreign keys). The vectors can be used to algebraically quantify semantic relationships between the tokens such as similarities and analogies. Vectors enable a dual view of the data: relational and (meaningful rather than purely syntactical) text. We introduce and explore a new class of queries called cognitive intelligence (CI) queries that extract information from the database based, in part, on the relationships encoded by vectors. We have implemented a prototype system on top of Spark to exhibit the power of CI queries. Here, CI queries are realized via SQL UDFs. This power goes far beyond text extensions to relational systems due to the information encoded in vectors. We also consider various extensions to the basic scheme, including using a collection of views derived from the database to focus on a domain of interest, utilizing vectors and/or text from external sources, maintaining vectors as the database evolves and exploring a database without utilizing its schema. For the latter, we consider minimal extensions to SQL to vastly improve query expressiveness.

==> background.tex <==
\section{Background: Distributed Representation using Word Vectors}

==> navigation.tex <==
% Explain that here we change SQL
% Explain the problem
% Explain how to extend SQL
% Show usage example (not implemented)
\subsection{Schema-less Navigation}
\label{sec:navigation}

In this section we consider extensions to SQL that  take advantage of the existence of vectors associated with database entities. 
The first extension is an ability to focus on individual entities within a field of a row. 
We add entities as "first class citizens"  by adding a phrase ‘Entity e’ in the FROM part of a SQL query.
We then extend SQL with the constructs (a) contains(column, entity),
(b) contains(row, entity), (c) contains(database, entity),(d)
cosineDistance(entity1, entity2)>c where entity, entity1 and entity2
are entity denoting variables or token constants and $c$ denotes a
constant $ -1.0 < c < 1.0$.   

The declaration \emph{Text entity e } declares $e$ to be a variable that can be bound to tokens. 
The statement \emph{contains(row, entity) } states that $entity$ must be bound to a token generated by tokenizing $row$.  If $entity$ is specified, e.g., \emph{contains(r, 'Physics')} then the result is TRUE for row $r$ whose tokenization includes the token 'Physics' and FALSE otherwise. The argument $column$ is specified by a relation name or alias followed by the column name as in 
\emph{contains(e.jobTitle, 'manager')} where $e$ is an alias for the emp relation. To indicate a whole row we use the star notation as in \emph{contains(e.*, 'manager')}.
The predicate$contains$ returns the number of occurrences TRUE means
bigger than zero. In fact, one can use it in expressions such as
\emph{contains(e.*, 'expert') > 1}.  

  
The ability to specify entities provides for a finer query
specification as compared to the UDFs we saw thus far. Relations may
be navigated using entities in a similar way as database keys. For
example, the following query checks for the existence of two strongly
related (cosine distance > 0.75)  entities in the address field of an
employee and a row (tuple) in the DEPT table (relation). 

\begin{figure}[htbp]
\hrule
{\small \tt{
\ix \\
SELECT EMP.Name, EMP.Salary, DEPT.Name \\
FROM EMP, DEPT, Entity e1, e2\\
WHERE contains(EMP.Address, e1) AND\\
contains(DEPT.*, e2) AND\\
cosineDistance(e1, e2) > 0.75\\
}
\hrule
}
\caption{Example of an SQL query with entities}
\label{fig:sql-entity}
\end{figure}



To enhance querying ability, we can proceed one step further and
introduce \emph{relation variables} whose names are not specified at
query writing time; they are identified at run-time via entities. 
Introducing relation variables is done as shown in the following
example.

\begin{figure}[htbp]
\hrule
{\small \tt{
\ix \\
SELECT EMP.Name, EMP.Salary, S.?1\\
FROM EMP, DEPT; Entity e1, e2; Relation S\\
WHERE contains(EMP.Address, e1) AND\\
contains(S.?1, e2) AND\\
cosineDistance(e1, e2) > 0.75 AND\\
contains(S.?1, e2) > 1  \\
}
\hrule
}
\caption{Example of an SQL query with relation variables}
\label{fig:sql-relation}
\end{figure}


In this example query, field (attribute) values are retrieved from EMP
and the (unknown) relation(s) S and column(s) ?1 such that there are
entities e1 and e2 that strongly "link" them. The “related” relation
and column names and the relevant values may also be
retrieved. Intuitively, we retrieve names and salaries from EMP and
tuple columns X out of some other relation S such that the
(tokenization of) tuple in EMP.Address contains an entity e1, the
(tokenization of) tuple in S's column X contains an entity e2 and e1
and e2 are "close" (cosine distance > 0.75) and has more than 1
occurrence of  entity e2. In general, there may be more than one
column in a qualifying relation that qualifies and there may be more
than one qualifying relation, and as such, the construct S.?1 should
indicate the relation and column names. For example, a result tuple
may look like: 
 \emph{(‘John Smith’, 112000, Dept.Mgr:‘Judy Smith’)}.  

The closeness  between entities may also be expressed qualitatively on
a scale, for example \emph{very\_strong, strong, moderate, weak,
  very\_weak}, e.g. \emph{strong(e1,e2)}. which enables defining the
numeric values separately, e.g. $very\_strong = 0.95$. For example,
understanding the relationship between the two entities ‘John’ and
'New York’ includes deriving the tokens for the  entities, in this
case simply 'John' and 'New York', locating their associated vectors,
say $V_John$ and $V_{New York}$, and performing an algebraic operation
on the two vectors, for example, calculating the cosine distance. If
the cosine distance between these vectors is high (i.e. closer to 1)
than the two entities are closely related; if the cosines distance is
low (i.e. closer to -1) the two entities are not closely related. 
 


==> operations.tex <==
%  Maintenance when DB changes
%  External text and DB sources
%  Externally supplied vectors
%  Various sets of vectors (of different dimensions), another parameter to choose when querying

\section{Operational Issues}
\label{sec:operations}

%The additional features are at the level of SQL additions which are in
%line with the “spirit” of SQL as well as additional built-in vector
%handling constructs. It is also possible to realize an embodiment
%described herein with no modification at all to SQL by (a) using User
%Defined Functions (UDFs), (b) having a standard relation called
%Vectors(key: String, Value: float Vector[0..m]) where the UDFs utilize
%the vectors and database fields to realize semantic querying.
%
%Exemplary embodiments  provide a user with a powerful and useful 'marriage' of machine
%learning technology and databases by embedding word vector technology
%into relational databases, as well as non-relational databases (e.g.,
%XML, RDF). The user may then query 'text entities' and their
%closeness. This extends current database capabilities that
%predominantly operate in the syntactic domain that is – computing
%numbers, comparing strings, finding sub-strings, counting string
%occurrences and using synonyms as the only semantic capability. The
%user may also navigate (join) a database without having a detailed
%knowledge of the schema, and query intelligently across different
%databases employing a different nomenclature. Embodiments described
%herein enable a user to intuitively and meaningfully query a database
%with terms that are not even mentioned in the database.

As the database evolves, the vectors need be updated. This can be done
by training anew every so often. Alternatively, or in conjunction, the
vectors may be maintained over time. The critical issue is the
introduction of new tokens (that do not have associated vectors). One
way of handling this is to first associate these with an 'average
vector' whose entries are very small (positive and negative)
values. Then, initiate training for a short duration (in the case of
word2vec) where the older vectors are not allowed to change (or, their
changes are multiplied by a very small positive fraction) and changes to
the new vectors are amplified. The net effect is that the new vectors
are assigned reasonable vector values. A detailed discussion of this
and similar techniques is deferred to a subsequent publication.


